Marginal Causal Flows for Validation and Inference

Investigating the marginal causal effect of an intervention on an outcome from complex data remains challenging due to the inflexibility of employed models and the lack of complexity in causal benchmark datasets, which often fail to reproduce intricate real-world data patterns. In this paper we introduce Frugal Flows, a novel likelihood-based machine learning model that uses normalising flows to flexibly learn the data-generating process, while also directly inferring the marginal causal quantities from observational data. We propose that these models are exceptionally well suited for generating synthetic data to validate causal methods. They can create synthetic datasets that closely resemble the empirical dataset, while automatically and exactly satisfying a user-defined average treatment effect. To our knowledge, Frugal Flows are the first generative model to both learn flexible data representations and also exactly parameterise quantities such as the average treatment effect and the degree of unobserved confounding. We demonstrate the above with experiments on both simulated and real-world datasets.

==> rebuttal_doc.tex <==
% % pageprob.tex  SE 560441
% \documentclass{book}
% %\documentclass{report}
% %\documentclass{article}
% \usepackage{url}            % simple URL typesetting
% \usepackage{booktabs}       % professional-quality tables
% \usepackage{amsfonts}       % blackboard math symbols
% \usepackage{amsmath,bm}
% \usepackage{dsfont}
% \usepackage{graphicx}
% \usepackage{caption}
% \usepackage{subcaption}
% \usepackage{color}
% \usepackage{nicefrac}       % compact symbols for 1/2, etc.
% \usepackage{microtype}      % microtypography
% \usepackage{xcolor}         % colors
% \usepackage{tikz}           % tikz
% \usepackage{array} % for better columns
% \usepackage{booktabs} % For professional looking tables
% \usepackage{cleveref}
% \usepackage{lipsum}
% \definecolor{pinegreen}{rgb}{0.0, 0.47, 0.44}
% % \usepackage[a4paper, total={8in, 12in}]{geometry}
% \usepackage[legalpaper, portrait, margin=0.15in]{geometry}
% \pagestyle{empty}
% \begin{document}
% \begin{table}[h!]
%     \centering
%     \caption{Mean and $2\sigma$ confidence interval of the inferred ATE for each model, bootstrapped over 25 different runs and with a data size of $N=25,\!000$. Bold confidence intervals contain the true ATE. OR quotes the results obtained by linear Outcome Regression, and CNF reports the ATE estimted by Causal Normalizing Flows.}
%     \begin{tabular}{l c c c c c c} % creating seven columns
%     \toprule %inserting double-line
%     Model & True ATE & Number of Covariates & Frugal Flow & OR & Matching & CNF \\ [0.5ex]
%     \toprule % inserts single-line
%     $M_{1}$ & $1$ & 4 & $\bm{0.98 \pm 0.12}$ & $1.28 \pm 0.06$ & $\bm{0.78 \pm 1.06}$ & $0.73 \pm 0.16$\\ 
%     $M_{1}$ & $5$ & 4 & $\bm{5.00 \pm 0.24}$ & $5.29 \pm 0.04$ & $\bm{4.68 \pm 1.06}$ & $4.23 \pm 0.20$\\ 
%     $M_{2}$ & $1$ & 4 & $\bm{1.01 \pm 0.10}$ & $1.46 \pm 0.07$ & $\bm{1.36 \pm 0.72}$ & $\bm{1.01 \pm 0.20}$\\
%     $M_{2}$ & $5$ & 4 & $\bm{5.01 \pm 0.18}$ & $5.44 \pm 0.05$ & $\bm{5.55 \pm 0.88}$ & $\bm{5.03 \pm 0.44}$\\
%     $M_{3}$ & $1$ & 10 & $ $ &  &  & $\bm{0.87 \pm 0.15}$\\
%     $M_{3}$ & $5$ & 10 &  & &  & $\bm{4.73 \pm 0.28}$\\
%     \bottomrule
%     \end{tabular}
%     \label{tab:sim-data-results}
% \end{table}

% \begin{table}[h!]
%     \centering
%     \caption{Version of CNF adding noise to discrete variables.}
%     \begin{tabular}{l c c c c } % creating seven columns
%     \toprule %inserting double-line
%     Model & True ATE & Number of Covariates & CNF \\ [0.5ex]
%     \toprule % inserts single-line
%     $M_{1}$ & $1$ & 4 & $0.52 \pm 0.05$\\ 
%     $M_{1}$ & $5$ & 4 & $4.36 \pm 0.19$\\ 
%     $M_{2}$ & $1$ & 4 & $0.71 \pm 0.16$ \\
%     $M_{2}$ & $5$ & 4 & $\bm{4.86 \pm 0.20}$ \\
%     $M_{3}$ & $1$ & 10 & $0.63 \pm 0.35$\\
%     $M_{3}$ & $5$ & 10 & $4.39 \pm 0.17$\\
%     \bottomrule
%     \end{tabular}
% \end{table}

% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=0.85\linewidth]{rebuttal_figures/Lalonde_NSW_0_1000_0.png}
%     \caption{\textbf{Lalonde} -- Correlation matrices across covariates and the outcome ($\texttt{re78}$) for comparing the second moments of distributions for the Lalonde observed real data and synthetic data generated by trained frugal flow and Credence (with default model settings ($3^{\text{rd}}$ column) and modified bias rigidity ($4^{\text{th}}$ column) models.}
%     \label{fig:lalonde-benchmark}
% \end{figure}
% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=0.85\linewidth]{rebuttal_figures/e401k_0_1000_0.png}
%     \caption{\textbf{e401(k)} -- Correlation matrices across covariates and the outcome ($\texttt{net\_tfa}$) for comparing the second moments of distributions for the e401(k) observed real data and synthetic data generated by trained frugal flow and Credence models.}
%     \label{fig:401k-benchmark}
% \end{figure}
% \begin{table}[h!]
%     \centering
%     \caption{$p$-values comparing the similarity between the original data and synthetic data generated using both frugal flows and Credence, for both the Lalonde and e401(k) datasets. Values higher than $p=0.05$ suggest that we do not have statistically significant evidence that the real and generated data come from different distributions.}
%     \begin{tabular}{l c c c c} % creating five columns
%     \toprule %inserting double-line
%     & \multicolumn{2}{c}{Lalonde} & \multicolumn{2}{c}{e401(k)} \\ 
%     \cmidrule(lr){2-3} \cmidrule(lr){4-5}
%     Method & Frugal Flows & Credence & Frugal Flows & Credence\\ [0.5ex]
%     \toprule % inserts single-line
%     MMD  & 0.36 & 0.00 & 0.98 & 0.00 \\ 
%     Energy  & 0.43 & 0.09 & 0.27 & 0.00 \\ 
%     FR & 0.06 & 0.00 & 0.34 & 0.00 \\ 
%     kNN  & 0.32 & 0.00 & 0.04 & 0.01 \\ 
%     \bottomrule
%     \end{tabular}
%     \label{tab:combined_pvals}
% \end{table}

% \begin{figure}[h!]
%     \centering
%     \begin{minipage}[t]{0.3\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{rebuttal_figures/dataset_sensitivity_plot.png}
%         \caption{Final ATE estimates from a trained frugal flow, with ATE parameter initialized at -10 (\color{red}red  line\color{black}), using data drawn from $M_{2}$ with a true ATE of 5 (\color{blue}blue line\color{black}). \color{pinegreen}Green dots\color{black}~ represent the final ATE the model converges on for each dataset size.}        
%         \label{fig:datasize_plot}
%     \end{minipage}
%     \hfill    
%     \begin{minipage}[t]{0.3\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{rebuttal_figures/lalonde_losses.png}
%         \caption{\color{blue}Training\color{black}~and \color{red}validation\color{black}~losses when fitting a frugal flow to the \textbf{Lalonde} dataset using optimal hyperparameters and a ``patience'' setting of 200 iterations for illustrative purposes.}
%         \label{fig:lalonde-log-likelihood}
%     \end{minipage}
%     \hfill
%     \begin{minipage}[t]{0.3\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{rebuttal_figures/e401k-loss.png}
%         \caption{\color{blue}Training\color{black}~and \color{red}validation\color{black}~losses when fitting a frugal flow to the \textbf{e401(k)} dataset using optimal hyperparameters and a ``patience'' setting of 200 iterations for illustrative purposes.}
%         \label{fig:e401k-log-likelihood}
%     \end{minipage}
% \end{figure}

% \end{document}
